PyramidCLIP: Hierarchical Feature Alignment for Vision-language Model Pretraining

Large-scale vision-language pre-training has achieved promising results on downstream tasks. Existing methods highly rely on the assumption that the image-text pairs crawled from the Internet are in perfect one-to-one correspondence. However, in real scenarios, this assumption can be difficult to hold: the text description, obtained by crawling the affiliated metadata of the image, often suffers from the semantic mismatch and the mutual compatibility. To address these issues, we introduce PyramidCLIP, which constructs an input pyramid with different semantic levels for each modality, and aligns visual elements and linguistic elements in the form of hierarchy via peer-level semantics alignment and cross-level relation alignment. Furthermore, we soften the loss of negative samples (unpaired samples) so as to weaken the strict constraint during the pre-training stage, thus mitigating the risk of forcing the model to distinguish compatible negative pairs. Experiments on five downstream tasks demonstrate the effectiveness of the proposed PyramidCLIP. In particular, with the same amount of 15 million pre-training image-text pairs, PyramidCLIP exceeds CLIP on ImageNet zero-shot classification top-1 accuracy by 10.6%/13.2%/10.0% with ResNet50/ViT-B32/ViT-B16 based image encoder respectively. When scaling to larger datasets, PyramidCLIP achieves the state-of-the-art results on several downstream tasks. In particular, the results of PyramidCLIP-ResNet50 trained on 143M image-text pairs surpass that of CLIP using 400M data on ImageNet zero-shot classification task, significantly improving the data efficiency of CLIP.

==> figures/enc.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width=9cm]{figures/enc.png}
    \caption{(a)~The schematic of CNN-based image encoder. (b)~The schematic of ViT-based image encoder. (c)~The structure of LeFF module in ViT.}
    \label{vitr50}
\end{figure}

==> figures/intro.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width=13.8cm]{figures/introimg.pdf}
    \caption{
    %Problems existing
    \textbf{Problems 
    in the web-crawled image-text pairs.} (a)(b)(c) suffer the semantic mismatch between visual modality and linguistic modality, while the image-text of (d) has similarities with the 
    unpaired text-image of (a). Note that, (a) the red caption is redundant, (b) the image outside the red bounding box is the redundant, (c) the descriptions for the casts in the red boxes are missing and the red caption in (d) is compatible with (a).
    }
    \label{introimg}
\end{figure}

==> tables/ablation_leff.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!htp]
\setlength{\belowcaptionskip}{1pt}
\centering
\caption{LEFF, YFCC15M, bs=4096, 8ep}
\begin{tabular}{c|cc|cc}
\toprule
\textbf{Method} & \textbf{Image Encoder}  & \textbf{IN ZS Top1} & \textbf{Image Encoder}  & \textbf{IN ZS Top1} \\ \hline 
%w/o LEFF(baseline)  &   34.7   \\ \hdashline
0  & VIT-B/16 &  35.8 & VIT-B/32 & 30.9\\
1  & VIT-B/16 &  36.6 & VIT-B/32 & 31.8\\
2  & VIT-B/16 &  36.9 & VIT-B/32 & 31.5\\
3  & VIT-B/16 &  37.3 & VIT-B/32 & 31.7\\
4  & VIT-B/16 &  38.3 & VIT-B/32 & 31.9\\ 
5  & VIT-B/16 &  38.4 & VIT-B/32 & 32.1\\ 
6  & VIT-B/16 &  38.3 & VIT-B/32 & 32.1\\ 
7  & VIT-B/16 &  38.4 & VIT-B/32 & 32.3\\ 
8  & VIT-B/16 &  38.4 & VIT-B/32 & 32.4\\ 
9  & VIT-B/16 &  38.6 & VIT-B/32 & 32.4\\
10 & VIT-B/16 &  38.5 & VIT-B/32 & 32.2\\ 
11 & VIT-B/16 &  38.7 & VIT-B/32 & 32.2 \\ 
12 & VIT-B/16 &  35.9 & VIT-B/32 & 29.2\\ 
\bottomrule
\end{tabular}
\end{table}

==> tables/ablation_object.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[!htp]
\setlength{\belowcaptionskip}{1pt}
\centering
\caption{Form of object contrast, YFCC15M, bs=4096, 8ep}
\begin{tabular}{c|ccc|ccc}
\toprule
\textbf{Method} & \textbf{Image Encoder} & \textbf{Top1} & \textbf{Top5} & \textbf{Image Encoder} & \textbf{Top1} & \textbf{Top5}\\ \hline 
w/o OC(baseline)  & ResNet50 &   34.7 & 60.6  & ViT-B/16 & 36.0 & 61.7 \\ \hdashline
Caption  & ResNet50 &   35.9  & 63.1  & ViT-B/16 &  38.6 & 65.2\\
Summ.    & ResNet50 &   36.2  & 62.2  & ViT-B/16 &  38.8 & 65.1 \\ 
Caption + Summ.  & ResNet50 &  \textbf{37.2}  & \textbf{63.9}   & ViT-B/16 & \textbf{39.6} & \textbf{66.1}\\ 
\bottomrule
\end{tabular}
\end{table}

==> tables/ablation_yfcc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[!htp]
% \setlength{\belowcaptionskip}{1pt}
% \centering
% \caption{Zero-shot accuracy on ImageNet. Ablation on YFCC15M, bs=4096, 8ep}
% \begin{tabular}{c|ccc|ccc}
% \toprule
% \textbf{Method} & \textbf{Image Encoder} & \textbf{Top1}  & \textbf{Top5}& \textbf{Image Encoder} & \textbf{Top1} & \textbf{Top5}\\ \hline 
% CLIP(baseline)  & ResNet50 &   29.2 & 53.6 & ViT-B/16 & 25.6 & 49.0 \\ \hdashline
% Local Contrast  & ResNet50 &   30.3 & 54.8 & ViT-B/16 & 27.3 & 50.7 \\
% + Global Contrast  & ResNet50 & 34.7 & 60.6 & ViT-B/16 &  32.6 & 58.3  \\ 
% + LEFF & ResNet50 & - & - & ViT-B/16 & 36.0 & 61.7 \\ 
% + Object Contrast & ResNet50 & \textbf{37.2} & \textbf{63.9} & ViT-B/16 &  \textbf{39.6} & \textbf{66.1}  \\ 
% \bottomrule
% \end{tabular}
% \end{table}


\begin{table}[!htp]
\setlength{\belowcaptionskip}{1pt}
\centering
\footnotesize
\caption{Ablation study of each component on ImageNet zero-shot classification task. $\mathcal{L}_{\rm CLIP}$ represents the original CLIP loss. ``LeFF''  represents the operation of incorporating depth-wise convolution into the FFN layer of ViT. ``Soften'' means that all the objectives are softened.}
\setlength{\tabcolsep}{1.0mm}{\begin{tabular}{cccccccc}
\toprule
\multirow{3}{*}[3pt]{\tabincell{c}{\textbf{Image}\\\textbf{Encoder}}} & \multicolumn{5}{c}{\textbf{Components}} & \multicolumn{2}{c}{\textbf{ImageNet}} \\
\cmidrule(r){2-6}\cmidrule(l){7-8}
  & $\mathcal{L}_{\rm intra}$ & LeFF & $\mathcal{L}_{\rm cross}^{\rm global}$ & $\mathcal{L}_{\rm cross}^{\rm local}$ &Soften & ZS Top1 & ZS Top5 \\ \midrule
\multirow{4}{*}{ResNet50} & \checkmark & -& & & & 32.8 & 58.5\\
& \checkmark&— & \checkmark& & &  & \\
& \checkmark&- &\checkmark &\checkmark & & 36.1(\textcolor{darkergreen}{+3.3}) & 63.0(\textcolor{darkergreen}{+4.5})\\ 
& \checkmark&- &\checkmark &\checkmark & \checkmark& \textbf{38.6(\textcolor{darkergreen}{+5.8})} & \textbf{64.8(\textcolor{darkergreen}{+6.3})}\\ 
\midrule
\multirow{5}{*}{ViT-B/32} & \checkmark & & & & & 28.8& 53.5\\
& \checkmark&\checkmark & & & & 29.7(\textcolor{darkergreen}{+0.9})&54.5(\textcolor{darkergreen}{+1.0})\\
&\checkmark&\checkmark & \checkmark& & & &\\
& \checkmark&\checkmark &\checkmark &\checkmark & &39.6(\textcolor{darkergreen}{+14.0})&66.1(\textcolor{darkergreen}{+17.1})\\
& \checkmark&\checkmark &\checkmark &\checkmark & \checkmark&\textbf{41.3(\textcolor{darkergreen}{+15.7})}&\textbf{68.1(\textcolor{darkergreen}{+19.1})}\\
\bottomrule
\end{tabular}}
\label{yfccablation}
\end{table}


% \begin{figure}
% \begin{minipage}[b]{.5\linewidth}
%     \centering
%     \includegraphics[width=5cm]{figures/enc.png}
%     \caption{.}
% \end{minipage}
% \begin{minipage}[b]{.5\linewidth} 
% \centering
% \captionof{table}{Table}
% \setlength{\tabcolsep}{0.5mm}{
% \begin{tabular}{c|cccccc|c}
% \toprule
% \textbf{Image Enc.} & $\mathcal{L}_{CLIP}$ & $\mathcal{L}_{LT}$ & $\mathcal{L}_{GS}$ & 
% DwFFN & $\mathcal{L}_{RT}$ & 
% $\mathcal{L}_{RS}$ & 
% \textbf{Top1} \\ 
% \hline 
% \multirow{4}{*}{ResNet50} &  &  & & & & & \\
% &  &  & & & & & \\
% &  &  & & & & & \\
% &  &  & & & & & \\
% \hline
% \multirow{4}{*}{ViT-B/16} &  &  & & & & & \\
% &  &  & & & & & \\
% &  &  & & & & & \\
% &  &  & & & & & \\
% \bottomrule
% \end{tabular}}
% \end{minipage}
% \end{figure}





==> tables/datasets.tex <==
\begin{table}[hb]
\caption{Pre-training datasets.}
\setlength{\tabcolsep}{1mm}{
\begin{tabular}{c|cccccc|c}
\hline
\textbf{Datasets} & SBU~\cite{ordonez2011im2text} & CC3M~\cite{sharma2018conceptual}  & CC12M~\cite{changpinyo2021conceptual}  &
YFCC15M-V1~\cite{thomee2016yfcc100m} & YFCC15M-V2~\cite{li2021supervision} & LAION99M~\cite{schuhmann2021laion} & Total \\ \hline
\textbf{\#$\langle$Image, Text$\rangle$ Pair} & 1M  & 3M  & 10M  & 15M & 15M & 99M  & 143M \\ \hline
%\bottomrule
\end{tabular}}
\label{pretrainingdata}
\end{table}



==> tables/linearprob.tex <==
\begin{table}[htp]
\setlength{\belowcaptionskip}{1pt}
\centering
\footnotesize
\caption{Linear Probe.}
\setlength{\tabcolsep}{0.9mm}{
\begin{tabular}{ccccccccccccccc}
\toprule
\textbf{Method} & \textbf{\tabincell{c}{\textbf{Pre-train} \\ \textbf{Dataset}}} &  \textbf{PET}& \textbf{C10} & \textbf{C100} & \textbf{DTD} & \textbf{CARS} &  \textbf{F101} & \textbf{FLOW} & \textbf{Air} & \textbf{SUN} & \textbf{CAL} &\textbf{IN} &\textbf{AVG}\\ 
\midrule
\multicolumn{3}{l}{\textit{\textbf{Image Encoder: ResNet50}}} & & & & \\
CLIP  &   400M  & 85.1 &  88.7  &  70.3 & 76.4 & 78.3 & 86.4 & 96.1 & 49.1 & 73.3 & 89.6 & 73.3 &  78.8   \\ 
DECLIP  &  88M  & 88.7 &  89.8  &  71.2 &  76.8 &  81.7 & 82.7 & 99.2 & 48.4 & 72.8 & 93.9 & 74.0 &  79.9  \\ 
\specialrule{0em}{1pt}{1pt}
CLIP$\Diamond$  & 143M & 82.9 & 84.5  & 64.5 & 74.3 & 79.3 & 80.5 & 93.2 & 45.4 & & & 71.2  \\ 
\textbf{PyramidCLIP}  &  143M & 87.8 & \textbf{91.8} &  \textbf{75.6} & 75.8 & \textbf{81.8} & 81.9 & 93.0 & \textbf{53.1} & \textbf{76.1} & \textbf{94.2}  & \textcolor{blue}{72.8} & \textbf{\textcolor{blue}{80.3}} \\ \hdashline
\multicolumn{3}{l}{\textit{\textbf{Image Encoder: ViT-B/32}}} & & & & \\
CLIP  &   400M   & 85.3 & 95.1  &  80.5  & 76.5 &  81.8 & 88.8 & 96.9 & 52.0 & 76.6 & 93.0 &  76.1 & 81.7    \\
DECLIP  &  88M   & 90.0 & 96.5  &  84.7  & 78.5 & 81.6  & 85.0  & 99.1 & 53.5 & 75.0 & 94.8 & 75.3 & 83.0    \\
CLIP$\Diamond$  & 143M  & 83.6 & 95.6  &  81.7 & 75.1 & 79.2 & 82.3 & 92.6 & 46.0 & & & 73.0 \\
\textbf{PyramidCLIP} & 143M  & 87.9 & 95.9 & 82.4 & 76.9 & \textbf{82.2} & 83.1& 93.0 & 50.3 & \textcolor{blue}{76.1} & 95.7 & 74.7 & \textcolor{blue}{81.7} \\ 
\bottomrule
\specialrule{0em}{1pt}{1pt}
\multicolumn{6}{l}{\small $\Diamond$ Our Implementation}
\end{tabular}}
\label{comparisononyfcc2}
\end{table}

==> tables/linearprobe_againstssl.tex <==
\begin{table}[htp]
\footnotesize
\setlength{\belowcaptionskip}{1pt}
\centering
\caption{Linear Probe against supervised and self-supervised approaches. INIK denotes ImageNet-1k.}
\begin{tabular}{ccccc}
\toprule
\textbf{Method} &  \textbf{\tabincell{c}{\textbf{Pre-train} \\ \textbf{Dataset}}} &  \textbf{Cifar-10} & \textbf{Cifar-100} & \textbf{ImageNet}\\ 
\midrule
\multicolumn{2}{l}{\textit{\textbf{Supervised Approaches}}} & & & \\
-  &  IN1K & 90.5 & 73.5  &  74.1   \\
%-  & ResNet50 &  IN21K &   &    &     \\
\hdashline
\multicolumn{2}{l}{\textit{\textbf{Self-supervised Approaches}}} & &  \\
DINO  &  IN1K   & \textbf{92.7}  & \textbf{76.8}   &  72.3     \\
DINO$\Diamond$  &   CC12M   &  82.5  &  60.4   &  61.7    \\
DINO$\Diamond$  &   YFCC15M-V1   &  80.9  &  59.1   & 61.8  \\
MoCo-v2(200ep) &    IN1K   &  91.2  &  72.5   &    61.3    \\
\hdashline
\multicolumn{2}{l}{\textit{\textbf{Vision-language Pre-training}}} & &  \\
\textbf{PyramidCLIP}  &  143M & \textbf{91.8}  &  \textbf{75.6} & \textbf{81.3}  \\ 
\bottomrule
\specialrule{0em}{1pt}{1pt}
\multicolumn{5}{l}{\small $\Diamond$ Our Implementation}
\end{tabular}
\label{comparisononyfcc2}
\end{table}

==> tables/objectdection_againstssl.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[htp]
\setlength{\belowcaptionskip}{1pt}
\centering
\caption{Object detection results on the VOC07 test with ResNet-50 backboned C4 based Faster R-CNN.}
\begin{tabular}{ccccc}
\toprule
\multirow{3}{*}[3pt]{\textbf{Method}} & \multirow{3}{*}[3pt]{\tabincell{c}{\textbf{Pre-train Dataset}}} & \multicolumn{3}{c}{\textbf{PASCAL VOC}}   \\ 
\cmidrule{3-5}
  & & $AP^{bb}$ & $AP^{bb}_{50}$ & $AP^{bb}_{75}$ \\ 
\midrule
\specialrule{0em}{2pt}{2pt}
\multicolumn{2}{l}{\textit{\textbf{Supervised Approaches}}} & & & \\
-  &  IN1K   &   51.4  &  78.4  &    56.4 \\
\hdashline
\multicolumn{2}{l}{\textit{\textbf{Self-supervised Approaches}}} \\
DINO  &  IN1K   &  42.2  & 74.3  &  42.2   \\ 
MoCo  &  IN1K   &    &   &     \\ 
DINO  &  CC12M  &    &   &     \\
DINO  &  YFCC15M-V1  &    &   &     \\
\specialrule{0em}{1pt}{1pt} 
\hdashline
\multicolumn{2}{l}{\textit{\textbf{Vision-language Pre-training}}} \\
CLIP$\Diamond$  &  400M  &  46.8   &  74.9  &  49.5   \\
\textbf{PyramidCLIP}   &  143M  &  \textbf{49.7}(\textcolor{darkergreen}{+2.9})   &  \textbf{77.7}(\textcolor{darkergreen}{+2.8})  &  \textbf{53.3}(\textcolor{darkergreen}{+3.8})   \\
\bottomrule
\specialrule{0em}{1pt}{1pt}
\multicolumn{5}{l}{\small $\Diamond$ Our Implementation}
\end{tabular}
\label{objectdetectionagainstssl}
\end{table}

==> tables/objectdetection.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[htp]
\setlength{\belowcaptionskip}{1pt}
\centering
\caption{Object detection results on the VOC07 test with ResNet50 backboned C4 based Faster R-CNN.}
\begin{tabular}{ccccc}
\toprule
\multirow{3}{*}[3pt]{\textbf{Method}} & \multirow{3}{*}[3pt]{\tabincell{c}{\textbf{Pre-train Dataset}}} & \multicolumn{3}{c}{\textbf{PASCAL VOC}}   \\ 
\cmidrule{3-5}
  & & \textbf{$AP^{bb}$} & \textbf{$AP^{bb}_{50}$} & \textbf{$AP^{bb}_{75}$} \\ 
\midrule
\multicolumn{2}{l}{\textit{\textbf{Random Initialized}}} & & & \\
— & — & 26.5 & 51.6 & 22.8 \\
\midrule
\specialrule{0em}{2pt}{2pt}
\multicolumn{2}{l}{\textit{\textbf{Comparison against SOTA Approaches}}} & & & \\
CLIP~\cite{radford2021learning}  &  400M   &  45.5   &  73.5  &  47.9   \\
DECLIP~\cite{li2021supervision}  &  88M    &  50.0   &  77.4  &  53.6   \\
\textbf{PyramidCLIP}   &   143M  &  \textbf{50.9}   &  \textbf{78.7}   &  \textbf{54.7}  \\
\midrule
\multicolumn{2}{l}{\textit{\textbf{Fair Comparison against CLIP}}} & & & \\
\specialrule{0em}{1pt}{1pt}
CLIP$\Diamond$  &  YFCC15M-V1   &   46.0  & 74.0   &  48.2   \\ 
\textbf{PyramidCLIP}   &  YFCC15M-V1   &  \textbf{49.8}(\textcolor{darkergreen}{+3.8})   &  \textbf{77.7}(\textcolor{darkergreen}{+3.7})  &  \textbf{53.5}(\textcolor{darkergreen}{+5.3})   \\ 
\hdashline
%CLIP$\Diamond$  &  YFCC15M-V2   &     &    &     \\ 
%\textbf{PyramidCLIP}   &  YFCC15M-V2   &  \textbf{}(\textcolor{darkergreen}{+})   &  \textbf{77.1}(\textcolor{darkergreen}{+})  &  \textbf{}(\textcolor{darkergreen}{+})   \\
%\hdashline
CLIP$\Diamond$  &  LAION15M  &  46.8   &  74.9  &  49.5   \\
\textbf{PyramidCLIP}   &  LAION15M  &  \textbf{49.7}(\textcolor{darkergreen}{+2.9})   &  \textbf{77.7}(\textcolor{darkergreen}{+2.8})  &  \textbf{53.3}(\textcolor{darkergreen}{+3.8})   \\
%CLIP$\Diamond$  &  TOTAL143M  &    &    &     \\
\bottomrule
\specialrule{0em}{1pt}{1pt}
\multicolumn{5}{l}{\small $\Diamond$ Our Implementation}
\end{tabular}
\label{objectdetection}
\end{table}

==> tables/objectdetection_ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[htp]
\setlength{\belowcaptionskip}{1pt}
\centering
\caption{Object detection results on the VOC07 test with ResNet-50 backboned C4 based Faster R-CNN.}
\begin{tabular}{ccccc}
\toprule
\multirow{3}{*}[3pt]{\textbf{Method}} & \multirow{3}{*}[3pt]{\tabincell{c}{\textbf{Pre-train Dataset}}} & \multicolumn{3}{c}{\textbf{PASCAL VOC}}   \\ 
\cmidrule{3-5}
  & & $AP^{bb}$ & $AP^{bb}_{50}$ & $AP^{bb}_{75}$ \\ 
\midrule
\specialrule{0em}{2pt}{2pt}
\multicolumn{2}{l}{\textit{\textbf{Ablation on YFCC15M, 8ep}}} & & & \\
\specialrule{0em}{1pt}{1pt}
CLIP$\Diamond$  &  YFCC15M-V1   &  44.6   &  73.4  &  46.9   \\
\textbf{PyramidCLIP} (w/o Relation) & YFCC15M-V1  &  45.6(\textcolor{darkergreen}{+1.0})   &  74.3(\textcolor{darkergreen}{+0.9})   &  47.7(\textcolor{darkergreen}{+0.8})    \\
\textbf{PyramidCLIP} & YFCC15M-V1  &  \textbf{47.0}(\textcolor{darkergreen}{+2.4})   &  \textbf{75.6}(\textcolor{darkergreen}{+2.2})   &  \textbf{50.4}(\textcolor{darkergreen}{+2.7})   \\ 

\bottomrule
\specialrule{0em}{1pt}{1pt}
\multicolumn{5}{l}{\small $\Diamond$ Our Implementation}
\end{tabular}
\label{objectdetectionagainstssl}
\end{table}

==> tables/sota-imagenet.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
%\begin{table}[htp]
%\setlength{\belowcaptionskip}{1pt}
%\centering
%\begin{tabular}{c|cc|cc}
%\toprule
%\textbf{Method} & \textbf{\#<Image, Text> Pair} &  \textbf{Image Encoder}  & \textbf{Top1 Acc} & %\textbf{Top5 Acc} \\  \hline
%CLIP            &  400M   &     ResNet50    &    59.6     &    —     \\ 
%CLIP            &  400M   &     ViT-B/32    &    63.2     &    —     \\ 
%CLIP            &  400M   &     ViT-B/16    &    68.6        &    —     \\ 
%DeCLIP          &  88M    &     ViT-B/32    &    66.2     &          \\
%FILIP           &  340M   &     ViT-B/32    &    68.8     &         \\ \hdashline
%CLIP(our imp.)  &  100M   &     ViT-B/16    &         &          \\ 
%CLIP(our imp.)  &  100M   &     ViT-B/32    &         &          \\ 
%Ours            &  100M   &                 &         &          \\ 
%\bottomrule
%\end{tabular}
%\end{table}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[htp]
\setlength{\belowcaptionskip}{1pt}
\centering
\caption{Zero-shot top1 accuracy on ImageNet. All models are pre-trained on large-scale dataset.}
\begin{tabular}{ccccc}
\toprule
\multirow{3}{*}[3pt]{\textbf{Method}} & \multirow{3}{*}[3pt]{\tabincell{c}{\textbf{Image}\\\textbf{Encoder}}} & \multicolumn{2}{c}{\textbf{Pre-training Setting}}  & \textbf{ImageNet}  \\  
\cmidrule{3-4}
                    &      & \# $\langle$Image, Text$\rangle$ Pair & Epoch  & ZS Top1  \\ 
\midrule
CLIP~\cite{radford2021learning}            &  ResNet50   &     400M    &   32  &    59.6   \\ 
DECLIP~\cite{li2021supervision}          &  ResNet50   &     88M     &   32  &    62.5   \\ 
\hdashline
CLIP$\Diamond$  &  ResNet50   &     128M    &   8   &    53.0   \\ 
\textbf{PyramidCLIP}   &  ResNet50   &     128M    &   8   &    57.7(\textcolor{darkergreen}{+4.7})   \\ \midrule
CLIP~\cite{radford2021learning}            &  ViT-B/32   &     400M    &   32  &    63.2   \\ 
DECLIP~\cite{li2021supervision}          &  ViT-B/32   &     88M     &   32  &    66.2   \\ 
FILIP~\cite{yao2021filip}           &  ViT-B/32   &     340M    &   30  &    68.8   \\ 
CLIP$\Diamond$  &  ViT-B/32   &     128M    &   32   &   55.5   \\ 
\hdashline
CLIP$\Diamond$  &  ViT-B/32   &     128M    &   8   &    49.7   \\ 
\textbf{PyramidCLIP}   &  ViT-B/32   &     128M    &   8   &    56.5(\textcolor{darkergreen}{+6.8})   \\
%CLIP            &  ViT-B/16   &     400M    &   32  &    68.6   \\ \hdashline
%CLIP(our imp.)  &  ViT-B/16   &     128M    &   8   &           \\ 
%\textbf{RMSC}   &  ViT-B/16   &     128M    &   8   &           \\
\midrule
CLIP~\cite{radford2021learning}            &  ViT-B/16   &     400M    &   32  &    68.6   \\ \hdashline
CLIP$\Diamond$  &  ViT-B/16   &     128M    &   8   &    54.4   \\ 
\textbf{PyramidCLIP}   &  ViT-B/16   &     128M    &   8   &    62.4(\textcolor{darkergreen}{+8.0})   \\

\bottomrule
\specialrule{0em}{1pt}{1pt}
\multicolumn{5}{l}{\small $\Diamond$ Our Implementation}
\end{tabular}
\label{sotaimagenet}
\end{table}

==> tables/tabY15.tex <==




%
% \begin{wrapfigure}{r}{1\textwidth}
%
%\vspace{-25pt}
\begin{table} 
\captionof{table}{Zero-shot top-1 accuracy on ImageNet. All the models are pre-trained for 32 epochs.}
% 
% \vspace{-5pt}
%
\makeatletter\def\@captype{table}
% \small
\centering
\setlength{\tabcolsep}{1mm}{\begin{tabular}{ccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \textbf{Image} &  \textbf{ImageNet} \\  
  & \textbf{Encoder} & ZS Top1  \\ 
\midrule
\specialrule{0em}{2pt}{2pt}
\multicolumn{3}{l}{\textit{\textbf{Pre-trained on YFCC15M-V2}}}\\
\specialrule{0em}{1pt}{1pt}
CLIP & ResNet50 & 37.2   \\
SLIP\cite{mu2021slip} & ResNet50 & 28.5   \\
FILIP & ResNet50 & 21.3   \\
DECLIP & ResNet50 & 41.9   \\
\hdashline
CLIP & ViT-B/32 & 32.8   \\ 
SLIP\cite{mu2021slip} & ViT-B/32 & 34.3  \\
\midrule
\specialrule{0em}{2pt}{2pt}
\multicolumn{3}{l}{\textit{\textbf{Pre-trained on YFCC15M-V1}}}\\
\specialrule{0em}{1pt}{1pt}
CLIP$\Diamond$ & ResNet50 & 25.5   \\ 
\textbf{PyramidCLP} & ResNet50 &   \textbf{44.7}   \\ 
\hdashline
CLIP$\Diamond$ & ViT-B/32 & 22.9  \\
%FILIP           & ViT-B/32 &  33.4   &   60.1  &   23.0  &   46.2  &   37.8   \\ 
DeFILIP & ViT-B/32 & 36.4  \\
\textbf{PyramidCLP} & ViT-B/32 & \textbf{41.4}  \\ 
\hdashline
CLIP$\Diamond$ & ViT-B/16 & 27.6  \\
\textbf{PyramidCLP} & ViT-B/16 &  \textbf{47.2}   \\
\bottomrule
\specialrule{0em}{1pt}{1pt}
\multicolumn{3}{l}{\small $\Diamond$ Our Implementation}
\end{tabular}}
% \vspace{-7pt}
\label{comparisononyfcc1}
\end{table} 



% \end{wrapfigure}




==> tables/transferabilitysmalldata.tex <==
\begin{table}[htp]
\setlength{\belowcaptionskip}{1pt}
\centering
\footnotesize
\caption{Accuracy on 10 datasets with ResNet50 image encoder. \textcolor{red}{C10/100/F101/FLOW/CAL/AIR is CIFAR10/C100/Food101/Flowers/Caltech}. AVG represents average accuracy. $\Diamond$ denotes Our Implementation.}
\setlength{\tabcolsep}{0.9mm}{
\begin{tabular}{ccccccccccccccc}
\toprule
\textbf{Method} & \textbf{\tabincell{c}{\textbf{Pre-train} \\ \textbf{Dataset}}} &  \textbf{PETS} & \textbf{C10} & \textbf{C100} & \textbf{DTD} & \textbf{CARS} &  \textbf{F101} & \textbf{FLOW} & \textbf{AIR} & \textbf{SUN} & \textbf{CAL} &\textbf{AVG}\\ 
\midrule
\multicolumn{3}{l}{\textit{\textbf{Zero-shot}}} & & & & \\
CLIP  &   400M   & \textbf{85.4} & 75.6 & 41.6 & 41.7 & 55.8 & \textbf{81.1} & \textbf{65.9} & \textbf{19.3} & 59.6 & \textbf{82.1}  & 60.8    \\
CLIP$\Diamond$  & 143M  & 77.0 & 56.4 & 26.7 & 41.4 & 54.6 & 69.8 & 60.4 & 7.3 & 60.6 & 76.1 & 53.6 \\
\textbf{PyramidCLIP} & 143M  & 83.7 & \textbf{81.5} & \textbf{53.7} & \textbf{47.2} & \textbf{65.0} & 67.8 & 65.8 & 12.6 & \textbf{65.8} & 81.7 & \textbf{62.4} \\ 
\hdashline
\multicolumn{3}{l}{\textit{\textbf{Linear Probe}}} & & & & \\
CLIP  &   400M  & 85.1 &  88.7  &  70.3 & 76.4 & 78.3 & \textbf{86.4} & 96.1 & 49.1 & 73.3 & 89.6  &  79.3   \\ 
DECLIP  &  88M  & \textbf{88.7} &  89.8  &  71.2 &  \textbf{76.8} &  81.7 & 82.7 & \textbf{99.2} & 48.4 & 72.8 & 93.9  &  80.5  \\ 
\specialrule{0em}{1pt}{1pt}
CLIP$\Diamond$  & 143M & 82.9 & 84.5  & 64.5 & 74.3 & 79.3 & 80.5 & 93.2 & 45.4 & 74.7 & 91.5 & 77.1  \\ 
\textbf{PyramidCLIP}  &  143M & 87.8 & \textbf{91.8} &  \textbf{75.6} & 75.8 & \textbf{81.8} & 81.9 & 93.0 & \textbf{53.1} & \textbf{76.1} & \textbf{94.2}  & \textbf{81.3} \\ 
\bottomrule
\specialrule{0em}{1pt}{1pt}
%\multicolumn{6}{l}{\small $\Diamond$ Our Implementation}
\end{tabular}}
\label{transfer2smallcls}
\end{table}
